Compatibility of $F$-isocrystals on adjoint Shimura varieties

In this article, we extend past results of the last two authors to include compatibility of canonical $\ell$-adic local systems and canonical $F$-isocrystals on adjoint Shimura varieties in the superrigid regime. Our method relies on the crystallinity of canonical $p$-adic local systems due to Esnault--Groechenig as well as Margulis superrigidity and the crystalline-to-\'etale companion construction of Drinfeld, Abe--Esnault, and Kedlaya.

==> mypreamble.tex <==

% Symbols
\usepackage{amsmath, amsthm, amssymb}
\usepackage{mathtools}
\usepackage{mathrsfs}  
\usepackage{stmaryrd}
\usepackage{comment}
\usepackage{marginnote}

% Style
\usepackage[margin=1in]{geometry}
\usepackage{parskip}
\usepackage[shortlabels]{enumitem}

% Colored text
%\usepackage{color}
\usepackage{xcolor}

% Links
\usepackage[bookmarks,colorlinks,breaklinks]{hyperref}
% PDF hyperlinks, with coloured links
\hypersetup{linkcolor=red,citecolor=blue,
  filecolor=dullmagenta,urlcolor=blue}

% Bibliography and references
\usepackage[numbers]{natbib}
\usepackage[capitalize]{cleveref}

% Figures
\usepackage{graphicx}
\usepackage{tikz}
\usetikzlibrary{matrix, arrows}
\usetikzlibrary{cd}

\NeedsTeXFormat{LaTeX2e}
\ProvidesPackage{quiver}[2021/01/11 quiver]

% `tikz-cd` is necessary to draw commutative diagrams.
\RequirePackage{tikz-cd}
% `amssymb` is necessary for `\lrcorner` and `\ulcorner`.
\RequirePackage{amssymb}
% `calc` is necessary to draw curved arrows.
\usetikzlibrary{calc}
% `pathmorphing` is necessary to draw squiggly arrows.
\usetikzlibrary{decorations.pathmorphing}

% A TikZ style for curved arrows of a fixed height, due to AndréC.
\tikzset{curve/.style={settings={#1},to path={(\tikztostart)
    .. controls ($(\tikztostart)!\pv{pos}!(\tikztotarget)!\pv{height}!270:(\tikztotarget)$)
    and ($(\tikztostart)!1-\pv{pos}!(\tikztotarget)!\pv{height}!270:(\tikztotarget)$)
    .. (\tikztotarget)\tikztonodes}},
    settings/.code={\tikzset{quiver/.cd,#1}
        \def\pv##1{\pgfkeysvalueof{/tikz/quiver/##1}}},
    quiver/.cd,pos/.initial=0.35,height/.initial=0}
\usepackage[all]{xy}
   \SelectTips{cm}{10}

\usepackage{hyperref}
\usepackage{enumitem}
\usepackage{graphicx}

\makeatletter
\def\thm@space@setup{%
  \thm@preskip=0.5em\thm@postskip=\thm@preskip%
}
\makeatother
% Unnamed theorem without counter
\newtheorem*{theorem}{Theorem}
\newtheoremstyle{named}{}{}{\\itshape}{}{\bfseries}{.}{.5em}{\thmnote{#3's }#1}
% Named theorem without counter
\theoremstyle{named}
\newtheorem*{namedtheorem}{Theorem}
% Other theorem environments
\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{claim}[thm]{Claim}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{sublem}[thm]{Sub-Lemma}
\newtheorem{cor}[thm]{Corollary}
\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{ex}[thm]{Exercise}
\newtheorem{eg}[thm]{Example}
\newtheorem{assumption}[thm]{Assumption}
\newtheorem{convention}[thm]{Convention}
\newtheorem{fact}{Fact}
\newtheorem{question}{Question}
\theoremstyle{remark}
\newtheorem{rmk}[thm]{Remark}
\crefformat{footnote}{#2\footnotemark[#1]#3}

%Hom
\newcommand{\Hom}{\mathrm{Hom}}

%Mathfrac
\newcommand{\fg}{\mathfrak{g}}

% Black board bold
\newcommand{\A}{\mathbb{A}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\Qlb}{\overline{\mathbb{Q}}_{\ell}}

%Algebraic groups
\newcommand{\GL}{\mathrm{GL}}
\newcommand{\SL}{\mathrm{SL}}
\newcommand{\SO}{\mathrm{SO}}
\newcommand{\OO}{\mathrm{O}}
\newcommand{\Sp}{\mathrm{Sp}}
\newcommand{\GSp}{\mathrm{GSp}}
\newcommand{\Spin}{\mathrm{Spin}}
\newcommand{\GSpin}{\mathrm{GSpin}}
\newcommand{\SU}{\mathrm{SU}}

%Trace
\newcommand{\tr}{\mathrm{tr}}

%Miscellaneous
\newcommand{\cO}{\mathcal{O}}

%Notational Shortcuts
\DeclareMathOperator{\Isoc}{Isoc}
\DeclareMathOperator{\Isocdag}{Isoc^\dagger}
\DeclareMathOperator{\Isocdagq}{Isoc^{(\dagger)}}
\DeclareMathOperator{\FIsoc}{\mathit{F}-Isoc}
\DeclareMathOperator{\FIsocdag}{\mathit{F}-Isoc^\dagger}
\DeclareMathOperator{\FIsocdagq}{\mathit{F}-Isoc^{(\dagger)}}
\DeclareMathOperator{\FaIsoc}{\mathit{F^a}-Isoc}
\DeclareMathOperator{\FaIsocdag}{\mathit{F^a}-Isoc^\dagger}
\DeclareMathOperator{\FaIsocdagq}{\mathit{F^a}-Isoc^{(\dagger)}}
\DeclareMathOperator{\IsocF}{Isoc_\textit{F}}
\DeclareMathOperator{\IsocdagF}{Isoc^\dagger_\textit{F}}
\DeclareMathOperator{\IsocdagqF}{Isoc^{(\dagger)}_\textit{F}}

\newcommand{\Gal}{\mathrm{Gal}}
\newcommand{\mf}{\mathfrak}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\ms}[1]{\mathscr{#1}}
\newcommand{\mr}[1]{\mathrm{#1}}
\newcommand{\mbb}[1]{\mathbb{#1}}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\ul}[1]{\underline{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\Ad}{\mathrm{Ad}}
\newcommand{\ad}{\mathrm{ad}}
\newcommand{\Frob}{\mathrm{Frob}}
%\renewcommand{\int}{\mathrm{int}}
\newcommand{\an}{\mathrm{an}}
\newcommand{\MIC}{\mathrm{MIC}}
\newcommand{\et}{\mathrm{\acute{e}t}}
\newcommand{\proet}{\mathrm{pro\acute{e}t}}
\newcommand{\Spec}{\mathrm{Spec}}
\newcommand{\Loc}{\mathrm{Loc}}
\newcommand{\Rep}{\mathrm{Rep}}
\renewcommand{\top}{\mathrm{top}}
\newcommand{\Sh}{\mathrm{Sh}}
\newcommand{\ltolp}{\lambda 
\rightsquigarrow \lambda'} %for companions
\newcommand{\Gad}{G^{\mathrm{ad}}}
\newcommand{\fgder}{\mathfrak{g}^{\mathrm{der}}}
\newcommand{\lf}{\mathrm{lf}}
\newcommand{\Vect}{\mathrm{Vect}}
\newcommand{\nilp}{\mathrm{nilp}}
\newcommand{\std}{\mathrm{std}}
\newcommand{\Fet}{\mathrm{F\acute{E}t}}


\DeclareMathOperator{\Aut}{Aut}
\DeclareMathOperator{\Out}{Out}
\DeclareMathOperator{\Res}{Res}
\DeclareMathOperator{\Pross}{Pro-ss}
\DeclareMathOperator{\im}{im}
\newcommand{\mat}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\DeclareMathOperator{\inn}{inn}
\DeclareMathOperator{\rec}{rec}
\DeclareMathOperator{\Nm}{Nm}
\DeclareMathOperator{\nil}{nil}
\DeclareMathOperator{\spect}{sp}
\newcommand{\ddt}{\frac{\partial}{\partial t}}

\newcommand{\tLS}{\widetilde{\LS}}
\newcommand{\git}{{\,\!\sslash\!\,}}
\newcommand{\dR}{\mathrm{dR}}
\newcommand{\alg}{\mathrm{alg}}
\newcommand{\perf}{\mathrm{perf}}
\newcommand{\Spa}{\mathrm{Spa}}
\newcommand{\Spf}{\mathrm{Spf}}
\newcommand{\Spd}{\mathrm{Spd}}
\newcommand{\FF}{\mathrm{FF}}
\renewcommand{\inf}{\mathrm{inf}}
\newcommand{\der}{\mathrm{der}}

\newcommand{\tor}{\mathrm{tor}}

\newcommand{\be}{\mathbf{e}}
\newcommand{\bv}{\mathbf{v}}

\newcommand{\pdif}[1]{\frac{\partial}{\partial #1}}
\newcommand{\VB}{\mathrm{VB}}
\newcommand{\Lie}{\mathrm{Lie}}
\newcommand{\dash}{\text{-}}

\newcommand{\wh}[1]{\widehat{#1}}


% p-adic Hodge theory
\newcommand{\crys}{\mathrm{crys}}
\newcommand{\logcrys}{{\mathrm{log}\text{-}\mathrm{crys}}}
\newcommand{\MF}{\mathrm{MF}}
\newcommand{\HdR}{\mathrm{HdR}}
\newcommand{\Fil}{\mathrm{Fil}}
\newcommand{\FilMIC}{\mathrm{FilMIC}}
\newcommand{\AR}{\mathrm{AR}}
\newcommand{\pMIC}{p\text{-}\mathrm{MIC}}


